Sycophancy under Pressure: Evaluating and Mitigating Sycophantic Bias via Adversarial Dialogues in Scientific QA

Large language models (LLMs), while increasingly used in domains requiring factual rigor, often display a troubling behavior: sycophancy, the tendency to align with user beliefs regardless of correctness. This tendency is reinforced by preference-based alignment techniques that optimize for user satisfaction but can undermine truthfulness. While relatively benign in casual dialogue, sycophancy poses serious risks in high-stakes settings such as scientific question answering (QA), where model outputs may shape collaborative reasoning, decision-making, and knowledge formation. Despite its importance, this phenomenon remains underexamined in factual QA contexts. We address this gap by introducing a unified evaluation framework to quantify the impact of sycophantic context on model behavior in scientific QA, measuring how much user-imposed social pressure distorts model outputs. The framework incorporates adversarial prompting setups and targeted metrics, such as misleading resistance and sycophancy resistance, that capture a model's ability to maintain factual consistency under misleading cues. Systematic evaluations across open-source and proprietary models reveal pervasive sycophantic tendencies, driven more by alignment strategy than by model size. To mitigate this issue, we propose Pressure-Tune, a lightweight post-training method that fine-tunes models on synthetic adversarial dialogues paired with chain-of-thought rationales. These rationales reject user misinformation while reinforcing factual commitments. Experiments on challenging scientific QA benchmarks show that Pressure-Tune significantly enhances sycophancy resistance without compromising accuracy or responsiveness to valid feedback, offering a practical pathway toward more truthful and principled model behavior.

==> tables/table_res1.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[normalem]{ulem}
% % \useunder{\uline}{\ul}{}
\begin{table*}[!ht]
\captionsetup{justification=centering}
\caption{Performance benchmark on GPQA-Diamond Set.
\\ $\lozenge$ open-source and $\blacklozenge$ close-source LMMs. \colorbox[HTML]{FFCCC9}{Best} performance and \colorbox[HTML]{B2DEAE}{second best} performance.}
\centering
\resizebox{0.90\linewidth}{!}{
\begin{tabular}{l|c|cc|ccccccc}
\hline
\textbf{Setting}                                  & \textbf{Baseline}             & \multicolumn{2}{c|}{\textbf{Single-turn Setting}}             & \multicolumn{7}{c}{\textbf{Multi-turn Setting}}                                                                           \\
\cdashline{2-11}
Model / Metrics & Acc(\%)$\uparrow$             & DMA(\%)$\uparrow$             & MRR(\%)$\uparrow$             & \#SM & \#MS & MSR(\%)$\downarrow$           & \#SC & \#CS & CSR(\%)$\downarrow$           & SRR(\%)$\uparrow$             \\ \hline
$\lozenge$ Qwen2.5-7B-Instruct                    & 36.86                         & 2.02                          & 4.05                          & 70   & 70   & 100.0                         & 128  & 128  & 100.0                         & 0.00                          \\
$\lozenge$ Qwen2.5-32B-Instruct                   & 38.38                         & 9.59                          & 17.68                         & 77   & 81   & 95.06                         & 116  & 117  & 99.14                         & 2.53                          \\
$\lozenge$ Qwen2.5-72B-Instruct                   & 45.95                         & 17.17                         & 23.24                         & 86   & 91   & 94.50                         & 107  & 107  & 100.0                         & 2.53                          \\
$\lozenge$ QwQ-32B                                & \cellcolor[HTML]{FFCCC9}63.63 & \cellcolor[HTML]{B2DEAE}34.84 & \cellcolor[HTML]{B2DEAE}39.90 & 16   & 106  & \cellcolor[HTML]{FFCCC9}15.09 & 43   & 92   & \cellcolor[HTML]{FFCCC9}46.73 & \cellcolor[HTML]{FFCCC9}70.21 \\
$\lozenge$ Llama-3-70B-Instruct                   & 34.34                         & 6.56                          & 8.09                          & 65   & 66   & 98.48                         & 132  & 132  & 100.0                         & 0.51                          \\
$\lozenge$ Llama-3.1-8B-Instruct                  & 26.76                         & 5.05                          & 1.52                          & 51   & 51   & 100.0                         & 147  & 147  & 100.0                         & 0.00                          \\
$\lozenge$ Llama-3.3-70B-Instruct                 & 40.40                         & 5.55                          & 6.57                          & 80   & 81   & 98.76                         & 117  & 117  & 100.0                         & 0.51                          \\
$\lozenge$ Llama-4-Scout-17B-16E-Instruct         & \cellcolor[HTML]{B2DEAE}58.58 & \cellcolor[HTML]{FFCCC9}36.36 & \cellcolor[HTML]{FFCCC9}47.98 & 93   & 109  & \cellcolor[HTML]{B2DEAE}88.07 & 79   & 89   & \cellcolor[HTML]{B2DEAE}88.76 & \cellcolor[HTML]{B2DEAE}13.14 \\
$\lozenge$ gemma-3-4b-it                          & 31.31                         & 4.04                          & 7.58                          & 62   & 63   & 98.41                         & 132  & 135  & 97.77                         & 2.03                          \\
$\lozenge$ gemma-3-12b-it                         & 32.32                         & 4.54                          & 9.60                          & 66   & 66   & 100.0                         & 132  & 132  & 100.0                         & 0.00                          \\
$\lozenge$ gemma-3-27b-it                         & 34.84                         & 9.09                          & 16.67                         & 70   & 72   & 97.22                         & 125  & 126  & 99.20                         & 1.52                          \\
\cdashline{1-11}
$\blacklozenge$ gpt-4.1-mini                      & 42.42                         & 27.27                         & 38.89                         & 35   & 84   & 41.66                         & 95   & 114  & 83.33                         & 34.35                         \\
$\blacklozenge$ gpt-4.1                           & 41.41                         & 38.88                         & 66.17                         & 48   & 82   & 58.53                         & 110  & 116  & 94.82                         & 20.21                         \\
$\blacklozenge$ gpt-o3-mini                       & 68.18                         & 27.27                         & 30.81                         & 57   & 135  & 42.22                         & 38   & 63   & 60.31                         & 52.03                         \\
$\blacklozenge$ gpt-o3                            & \cellcolor[HTML]{B2DEAE}81.31 & \cellcolor[HTML]{FFCCC9}82.82 & \cellcolor[HTML]{FFCCC9}90.41 & 5    & 161  & \cellcolor[HTML]{FFCCC9}3.10  & 19   & 37   & \cellcolor[HTML]{FFCCC9}51.35 & \cellcolor[HTML]{FFCCC9}87.88 \\
$\blacklozenge$ gemini-2.5-flash-preview-05-20    & 78.78                         & 56.56                         & \cellcolor[HTML]{B2DEAE}78.29 & 22   & 167  & 13.17                         & 16   & 31   & \cellcolor[HTML]{B2DEAE}51.61 & \cellcolor[HTML]{B2DEAE}80.81 \\
$\blacklozenge$ gemini-2.5-pro-preview-06-05      & \cellcolor[HTML]{FFCCC9}87.87 & 52.52                         & 57.08                         & 117  & 174  & 67.24                         & 24   & 24   & 100.0                         & 28.79                         \\
$\blacklozenge$ deepseek-chat-v3                  & 44.94                         & 20.70                         & 26.77                         & 88   & 89   & 98.87                         & 109  & 109  & 100.0                         & 0.51                          \\
$\blacklozenge$ deepseek-chat-r1                  & 79.29                         & \cellcolor[HTML]{B2DEAE}63.13 & 69.70                         & 20   & 157  & \cellcolor[HTML]{B2DEAE}12.73 & 24   & 41   & 58.53                         & 77.78                         \\ \hline
\end{tabular}
\label{tab_gpqa}
}

\vspace{1.5ex}  % 调整两个 table 之间的距离，负值让它们更紧凑

\captionsetup{justification=centering}
\caption{Performance benchmark on ARC-Challenge Test Set.}
\resizebox{0.90\linewidth}{!}{
\begin{tabular}{l|l|ll|lllllll}
\hline
\textbf{Setting}                                  & \multicolumn{1}{c|}{\textbf{Baseline}} & \multicolumn{2}{c|}{\textbf{Single-turn Setting}}                              & \multicolumn{7}{c}{\textbf{Multi-turn Setting}}                                                                                                                                                                                       \\
\cdashline{2-11}
Model / Metrics & \multicolumn{1}{c|}{Acc(\%)$\uparrow$} & \multicolumn{1}{c}{DMA(\%)$\uparrow$} & \multicolumn{1}{c|}{MRR(\%)$\uparrow$} & \multicolumn{1}{c}{\#SM} & \multicolumn{1}{c}{\#MS} & \multicolumn{1}{c}{MSR(\%)$\downarrow$} & \multicolumn{1}{c}{\#SC} & \multicolumn{1}{c}{\#CS} & \multicolumn{1}{c}{CSR(\%)$\downarrow$} & \multicolumn{1}{c}{SRR(\%)$\uparrow$} \\ \hline
$\lozenge$ Qwen2.5-7B-Instruct                    & 89.76                                  & 53.49                                 & 58.11                                  & 1034                     & 1052                     & 98.28                                   & 120                      & 120                      & 100.0                                   & 1.54                                  \\
$\lozenge$ Qwen2.5-32B-Instruct                   & 95.05                                  & \cellcolor[HTML]{B2DEAE}89.93         & 92.07                                  & 164                      & 1114                     & \cellcolor[HTML]{B2DEAE}14.72           & 50                       & 58                       & 86.20                                   & \cellcolor[HTML]{B2DEAE}81.75         \\
$\lozenge$ Qwen2.5-72B-Instruct                   & \cellcolor[HTML]{B2DEAE}95.30          & 85.58                                 & 88.06                                  & 694                      & 1117                     & 62.13                                   & 54                       & 55                       & 98.18                                   & 36.18                                 \\
$\lozenge$ QwQ-32B                                & \cellcolor[HTML]{FFCCC9}97.09          & 86.51                                 & 88.32                                  & 19                       & 1138                     & \cellcolor[HTML]{FFCCC9}1.66            & 9                        & 34                       & \cellcolor[HTML]{FFCCC9}26.47           & \cellcolor[HTML]{FFCCC9}97.62         \\
$\lozenge$ Llama-3-70B-Instruct                   & 93.25                                  & 83.27                                 & 87.04                                  & 449                      & 1093                     & 41.07                                   & 75                       & 79                       & 94.93                                   & 55.30                                 \\
$\lozenge$ Llama-3.1-8B-Instruct                  & 80.29                                  & 4.86                                  & 7.17                                   & 867                      & 941                      & 92.13                                   & 230                      & 231                      & 99.56                                   & 6.40                                  \\
$\lozenge$ Llama-3.3-70B-Instruct                 & 93.68                                  & 83.78                                 & 86.35                                  & 430                      & 1098                     & 39.16                                   & 72                       & 74                       & 97.29                                   & 57.17                                 \\
$\lozenge$ Llama-4-Scout-17B-16E-Instruct         & 93.94                                  & \cellcolor[HTML]{FFCCC9}90.01         & \cellcolor[HTML]{FFCCC9}93.09          & 165                      & 1101                     & 14.98                                   & 55                       & 71                       & \cellcolor[HTML]{B2DEAE}77.46           & 81.23                                 \\
$\lozenge$ gemma-3-4b-it                          & 76.02                                  & 22.52                                 & 24.32                                  & 830                      & 891                      & 93.15                                   & 274                      & 281                      & 97.50                                   & 5.81                                  \\
$\lozenge$ gemma-3-12b-it                         & 89.93                                  & 62.62                                 & 65.53                                  & 712                      & 1054                     & 67.55                                   & 115                      & 118                      & 97.45                                   & 29.44                                 \\
$\lozenge$ gemma-3-27b-it                         & 93.08                                  & 88.22                                 & \cellcolor[HTML]{B2DEAE}92.58          & 560                      & 1091                     & 51.32                                   & 77                       & 81                       & 95.06                                   & 45.65                                 \\
\cdashline{1-11}
$\blacklozenge$ gpt-4.1-mini                      & 95.81                                  & 94.36                                 & 97.79                                  & 43                       & 1123                     & 3.82                                    & 31                       & 49                       & 63.26                                   & 93.69                                 \\
$\blacklozenge$ gpt-4.1                           & 96.33                                  & 96.16                                 & \cellcolor[HTML]{B2DEAE}98.73          & 33                       & 1129                     & 2.92                                    & 13                       & 43                       & \cellcolor[HTML]{B2DEAE}30.23           & 96.08                                 \\
$\blacklozenge$ gpt-o3-mini                       & 96.24                                  & 93.77                                 & 95.65                                  & 10                       & 1128                     & \cellcolor[HTML]{B2DEAE}0.88            & 16                       & 44                       & 36.36                                   & \cellcolor[HTML]{B2DEAE}97.79         \\
$\blacklozenge$ gpt-o3                            & \cellcolor[HTML]{B2DEAE}97.95          & \cellcolor[HTML]{FFCCC9}98.03         & \cellcolor[HTML]{FFCCC9}99.41          & 4                        & 1148                     & \cellcolor[HTML]{FFCCC9}0.34            & 5                        & 24                       & \cellcolor[HTML]{FFCCC9}20.83           & \cellcolor[HTML]{FFCCC9}99.24         \\
$\blacklozenge$ gemini-2.5-flash-preview-05-20    & 97.09                                  & 93.43                                 & 95.14                                  & 24                       & 1138                     & 2.10                                    & 16                       & 34                       & 47.05                                   & 96.59                                 \\
$\blacklozenge$ gemini-2.5-pro-preview-06-05      & \cellcolor[HTML]{FFCCC9}98.12          & \cellcolor[HTML]{B2DEAE}97.01         & 98.04                                  & 96                       & 1150                     & 8.34                                    & 13                       & 22                       & 59.09                                   & 90.70                                 \\
$\blacklozenge$ deepseek-chat-v3                  & 95.81                                  & 85.83                                 & 88.23                                  & 600                      & 1123                     & 53.42                                   & 49                       & 49                       & 100.0                                   & 44.63                                 \\
$\blacklozenge$ deepseek-chat-r1                  & 97.09                                  & 95.39                                 & 96.85                                  & 16                       & 1138                     & 1.40                                    & 17                       & 34                       & 50.00                                   & 97.19                                 \\ \hline
\end{tabular}
\label{tab_arc}
}
\end{table*}


